Application of a Semi-automatic Algorithm for Identification of Molecular Components in SBML Models

Reactions forming a pathway can be rewritten by making explicit the different molecular components involved in them. A molecular component represents a biological entity (e.g. a protein) in all its states (free, bound, degraded, etc.). In this paper we show the application of a component identification algorithm to a number of real-world models to experimentally validate the approach. Components identification allows subpathways to be computed to better understand the pathway functioning.

==> eptcsdata.tex <==
\providecommand{\firstpage}{43}
\providecommand{\publicationstatus}{A. Graudenzi, G. Caravagna, G. Mauri, M. Antoniotti (Eds.): \\Wivace 2013 - Italian Workshop on \\Artificial Life and Evolutionary Computation\\
EPTCS 130, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.130.7}{10.4204/EPTCS.130.7}}
\pdfoutput=1

